First Light And Reionisation Epoch Simulations (FLARES) XIV: The Balmer/4000~\AA\ Breaks of Distant Galaxies

With the successful launch and commissioning of JWST we are now able to routinely spectroscopically probe the rest-frame optical emission of galaxies at $z>6$ for the first time. Amongst the most useful spectral diagnostics used in the optical is the Balmer/4000~\AA\ break; this is, in principle, a diagnostic of the mean ages of composite stellar populations. However, the Balmer break is also sensitive to the shape of the star formation history, the stellar (and gas) metallicity, the presence of nebular continuum emission, and dust attenuation. In this work we explore the origin of the Balmer/4000~\AA\ break using the SYNTHESIZER synthetic observations package. We then make predictions of the Balmer/4000~\AA\ break using the First Light and Reionisation Epoch Simulations (FLARES) at $5<z<10$. We find that the average break strength weakly correlates with stellar mass and rest-frame far-UV luminosity, but that this is predominantly driven by dust attenuation. We also find that break strength provides a weak diagnostic of the age but performs better as a means to constrain star formation and stellar mass, alongside the UV and optical luminosity, respectively.

==> Sections/app.tex <==
\section{Comparison of machine learning methods}\label{sec:first_appendix}

\subsection{Other methods}

We trialled two machine learning methods in addition to XGBoost -- Extremely Randomised Trees (ERT) and neural networks. For these models, our method for hyperparameter optimisation and model training was the same as that outlined in Section \ref{sec:ml.method}. To evaluate the usefulness of machine learning, we also obtained predictions for a simple model, fitted using linear least squares regression. 

\subsubsection{Extremely Randomised Trees}

Like XGBoost, Extremely Randomised Trees (ERT) is an ensemble method that combines the results of multiple CARTs. However, instead of generating trees sequentially, ERT averages the predictions of a large number of trees that have been trained independently. The split points of each tree are chosen randomly for each feature. We used the scikit-learn \cite[]{scikit-learn} implementation of ERT. The hyperparameters for each ERT model were obtained from the following hyperparameter grid: `min\_samples\_split': [10, 300, step=10], `min\_samples\_leaf': [10, 300, step=10], `n\_estimators': [10, 500, step=10].

\subsubsection{Neural Networks}

A neural network consists of layers of nodes. At each node, a mapping is performed using a specified activation function. The result of this mapping is passed to nodes in the subsequent layer, where the data is again transformed. Each connection between nodes is associated with a weight. Training a neural network involves adjusting these weights in order to reduce the loss. We used the Keras \cite[]{chollet2015keras} implementation of neural networks. For hyperparameter optimisation, we used the following grid: `neurons': [1, 30, step=1], `batch\_size': [25, 500, step=25], `epochs': [100, 1200, step=50], `n\_layers': [1, 20, step=1].

\subsubsection{Linear least squares regression}

The fitting function we use is a linear combination of the spectral diagnostics up to third order (we found that going to higher order than this leads to minimal improvement). To obtain predictions, the model was fitted using the training data, and the $R^2$ score was computed for the fitted model applied to the test data. The final $R^2$ score was averaged over a 5-fold cross-validation.

\subsection{Comparison}

We find that in general, the machine learning methods make better predictions than the fitting function we used. Of the three machine learning models, XGBoost performs marginally better for all physical properties, with the exception of stellar age. Although all three models performed similarly for the most part, the tree-based ensemble methods were quicker to optimise and train.

\begin{figure}
    \includegraphics[width=\columnwidth]{figs_LS/cubereg_ert_mlp_xgb_compare r2.png}
	\caption{$R^2$ values obtained for the three machine learning models (XGBoost, Extremely Randomised Trees, neural network). We also used linear least squares regression \label{fig:models_r2}}
\end{figure}
